Token-Level Inference-Time Alignment for Vision-Language Models

Vision-Language Models (VLMs) have become essential backbones of modern multimodal intelligence, yet their outputs remain prone to hallucination-plausible text misaligned with visual inputs. Existing alignment approaches often rely on expensive fine-tuning with annotated preference data or sequence-level inference strategies that provide only coarse, delayed feedback. To overcome these limitations, we present TITA (Token-level Inference-Time Alignment), a lightweight framework that freezes the base VLM and instead trains a reward model to approximate its distribution. During inference, implicit preference signals are extracted as log-probability ratios between the reward model and the target VLM, yielding dense autoregressive feedback. This formulation can be viewed as an inference-time variant of Direct Preference Optimization (DPO), providing token-level corrective signals without retraining the backbone. Extensive evaluations on LLaVA-1.5-7B and 13B show consistent gains across 12 benchmarks, with improvements of 8.6% on MMVet and 6.7% on POPE, indicating stronger general understanding and reduced hallucinations. Additional experiments on Qwen2.5-VL-7B and DeepSeek-VL2-27.5B show comparable gains, especially in hallucination reduction and VQA accuracy, while incurring negligible inference overhead.

==> notations.tex <==
% \newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
% \newtheorem{claim}{Claim}
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{assumption}{Assumption}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{fact}{Fact}[section]
% \theoremstyle{definition}
% \newtheorem{condition}{Condition}[section]
% \newtheorem{definition}{Definition}[section]
% \newtheorem{example}{Example}
% \theoremstyle{remark}
% \newtheorem{remark}{Remark}
% \newtheorem{discussion}{Discussion}[section]
% \newtheorem{fact}{Fact}[section]

\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{fact}{Fact}
% \theoremstyle{definition}
\newtheorem{condition}{Condition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
% \theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{discussion}{Discussion}

% Jamie bar commend
\makeatletter
\newsavebox\myboxA
\newsavebox\myboxB
\newlength\mylenA

\newcommand*\xbar[2][0.75]{%
    \sbox{\myboxA}{$\m@th#2$}%
    \setbox\myboxB\null% Phantom box
    \ht\myboxB=\ht\myboxA%
    \dp\myboxB=\dp\myboxA%
    \wd\myboxB=#1\wd\myboxA% Scale phantom
    \sbox\myboxB{$\m@th\overline{\copy\myboxB}$}%  Overlined phantom
    \setlength\mylenA{\the\wd\myboxA}%   calc width diff
    \addtolength\mylenA{-\the\wd\myboxB}%
    \ifdim\wd\myboxB<\wd\myboxA%
       \rlap{\hskip 0.5\mylenA\usebox\myboxB}{\usebox\myboxA}%
    \else
        \hskip -0.5\mylenA\rlap{\usebox\myboxA}{\hskip 0.5\mylenA\usebox\myboxB}%
    \fi}
\makeatother


% \newcommand{\theHalgorithm}{\arabic{algorithm}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\newcommand{\tens}[1]{\boldsymbol{\mathscr{#1}}}
\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\grad}{\nabla}
\newcommand{\hess}{\nabla^2}
\newcommand{\pgrad}[1]{ \frac{\partial}{\partial{#1} }}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\argsup}{\mathop{\rm argsup}}

\newcommand{\fft}{ \mbox{\tt fft} }
\newcommand{\ifft}{ \mbox{\tt ifft} }
\newcommand{\svd}{ \mbox{\tt svd} }

\newcommand{\Unif}{\textrm{Unif}}
\newcommand{\abs}[1]{\left|{#1}\right|}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\fnorm}[1]{\|{#1}\|_{\text{F}}}
\newcommand{\infnorm}[1]{\|{#1}\|_\infty}
\newcommand{\spnorm}[2]{\left\| {#1} \right\|_{\text{S}({#2})}}
\newcommand{\sigmin}{\sigma_{\min}}
\newcommand{\tr}{\text{tr}}
\newcommand{\defeq}{\stackrel{\textrm{def}}{=}}
\renewcommand{\det}{\text{det}}
\newcommand{\rank}{\text{rank}}
\newcommand{\logdet}{\text{logdet}}
\newcommand{\trans}{^{\top}}
\newcommand{\poly}{\text{poly}}
\newcommand{\polylog}{\text{polylog}}
\newcommand{\st}{\text{s.t.~}}
\newcommand{\proj}{\mathcal{P}}

\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rd}{\mathbb{R}^d}
\newcommand{\Rdd}{\mathbb{R}^{d\times d}}
\newcommand{\Var}{\text{Var}}

\newcommand{\expect}{\mathbb{E}}
\newcommand{\prob}{\mathbb{P}}


%%tensors X=L+E A=USV^H
\newcommand{\tA}{\tens{A}}
\newcommand{\tT}{\tens{T}}
\newcommand{\tB}{\tens{B}}
\newcommand{\tC}{\tens{C}}
\newcommand{\tX}{\tens{X}}
\newcommand{\tL}{\tens{L}}
\newcommand{\tE}{\tens{E}}
\newcommand{\tU}{\tens{U}}
\newcommand{\tV}{\tens{V}}
\newcommand{\tS}{\tens{S}}
\newcommand{\tVH}{\tens{V}^{\mathbf{H}}}
\newcommand{\tM}{\tens{M}}
\newcommand{\tJ}{\tens{J}}
\newcommand{\tG}{\tens{G}}
\newcommand{\tI}{\tens{I}}
\newcommand{\tQ}{\tens{Q}}

\newcommand{\tO}{\tens{O}}

\newcommand{\tY}{\tens{Y}}

\newcommand{\td}{{\tt D}_{\w\w}}
\newcommand{\tdv}{{\tt D}_{\v\v}}
% \newcommand{\htX}{\widehat{\tX}}
% \newcommand{\htY}{\widehat{\tY}}
% \newcommand{\htA}{\widehat{\tA}}
% \newcommand{\htB}{\widehat{\tB}}
% \newcommand{\htT}{\widehat{\tT}}
% \newcommand{\htL}{\widehat{\tL}}
% \newcommand{\htG}{\widehat{\tG}}
% \newcommand{\htU}{\widehat{\tU}}
% \newcommand{\htS}{\widehat{\tS}}
% \newcommand{\htV}{\widehat{\tV}}

% \newcommand{\htX}{\tX_\mathscr{F}}
% \newcommand{\htY}{\tY_\mathscr{F}}
% \newcommand{\htA}{\tA_\mathscr{F}}
% \newcommand{\htB}{\tB_\mathscr{F}}
% \newcommand{\htT}{\tT_\mathscr{F}}
% \newcommand{\htL}{\tL_\mathscr{F}}
% \newcommand{\htG}{\tG_\mathscr{F}}
% \newcommand{\htU}{\tU_\mathscr{F}}
% \newcommand{\htS}{\tS_\mathscr{F}}
% \newcommand{\htV}{\tV_\mathscr{F}}

\newcommand{\fracpar}[2]{\frac{\partial #1}{\partial  #2}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

% \newcommand{\A}{\mat{A}}
% \newcommand{\B}{\mat{B}}
% \newcommand{\C}{\mat{C}}
% \renewcommand{\S}{\mat{S}}
% \newcommand{\I}{\mat{I}}
% \newcommand{\M}{\mat{M}}
% \newcommand{\D}{\mat{D}}
% \renewcommand{\P}{\mat{P}}
% \newcommand{\mQ}{\mat{Q}}
% \newcommand{\mR}{\mat{R}}


% \newcommand{\U}{\mat{U}}
% \newcommand{\V}{\mat{V}}
% \newcommand{\W}{\mat{W}}
\newcommand{\X}{\mat{X}}
% \newcommand{\Y}{\mat{Y}}
% \newcommand{\mZ}{\mat{Z}}
% \newcommand{\mSigma}{\mat{\Sigma}}
% \newcommand{\G}{\mat{G}}

% \newcommand{\mU}{\mat{U}}
% \newcommand{\mV}{\mat{V}}
\renewcommand{\S}{\mat{S}}

\renewcommand{\O}{\mat{O}}
\newcommand{\Q}{\mat{Q}}
\newcommand{\E}{\mat{E}}
\renewcommand{\H}{\mat{H}}

%%matrices X=L+E
% \newcommand{\mX}{\mat{X}}
% \newcommand{\mL}{\mat{L}}
% \newcommand{\mE}{\mat{E}}
% \newcommand{\mM}{\mat{M}}
% \newcommand{\mA}{\mat{A}}
% \newcommand{\mB}{\mat{B}}
% \newcommand{\mC}{\mat{C}}
% \newcommand{\mT}{\mat{T}}
% \newcommand{\mY}{\mat{Y}}

% %%matrices bar X=L+E
% \newcommand{\bmX}{\xbar{\mX}}
% \newcommand{\bmL}{\xbar{\mL}}
% \newcommand{\bmE}{\xbar{\mE}}
% \newcommand{\bmM}{\xbar{\mM}}
% \newcommand{\bmA}{\xbar{\mA}}

% \newcommand{\bmY}{\xbar{\mY}}
% \newcommand{\bmU}{\xbar{\U}}
% \newcommand{\bmV}{\xbar{\V}}
% \newcommand{\bmG}{\xbar{\G}}

% \newcommand{\hmM}{\widehat{\mM}}
% \newcommand{\hmY}{\widehat{\mY}}
% \newcommand{\hmA}{\widehat{\mA}}
% \newcommand{\hmU}{\widehat{\U}}
% \newcommand{\hmV}{\widehat{\V}}
% \newcommand{\hmB}{\widehat{\mB}}
% \newcommand{\hmT}{\widehat{\mT}}
% \newcommand{\hmG}{\widehat{\G}}


% \newcommand{\hmM}{\mM_\mathscr{F}}
% \newcommand{\hmY}{\mY_\mathscr{F}}
% \newcommand{\hmA}{\mA_\mathscr{F}}
% \newcommand{\hmU}{\U_\mathscr{F}}
% \newcommand{\hmV}{\V_\mathscr{F}}
% \newcommand{\hmB}{\mB_\mathscr{N}}
% \newcommand{\hmT}{\mT_\mathscr{F}}
% \newcommand{\hmG}{\G_\mathscr{F}}


\newcommand{\vectsigma}{\bm{\sigma}}

\newcommand{\FU}{F_{S^{\setminus}}}
\newcommand{\FS}{F_{S}}
\newcommand{\WF}{\widetilde F}
\newcommand{\WFS}{\widetilde F_{S}}
\newcommand{\WFU}{\widetilde F_{S^{\setminus}}}

\newcommand{\mLambda}{\mat{\Lambda}}
\newcommand{\e}{\vect{e}}
\renewcommand{\u}{\vect{u}}
\renewcommand{\v}{\bm{\nu}}
\newcommand{\vt}{\bm{\nu}_{t}}
\newcommand{\vtpp}{\bm{\nu}_{t+1}}
\newcommand{\p}{\vect{p}}
\newcommand{\g}{\vect{g}}
\renewcommand{\a}{\vect{a}}
\newcommand{\w}{\bm{\omega}}

\renewcommand{\wp}{\bm{\omega}_P^*}
\newcommand{\wn}{\bm{\omega}_{S}^*}
\newcommand{\wnu}{\bm{\omega}_{S^{\setminus}}^*}
\newcommand{\hw}{\widehat{\w}}
\newcommand{\hwu}{\widehat{\w}_{S^{\setminus}}}
\newcommand{\hv}{\widehat{\v}}
\newcommand{\hvu}{\widehat{\v}_{S^{\setminus}}}
\newcommand{\tw}{\widetilde{\w}}
\newcommand{\tv}{\widetilde{\v}}
\newcommand{\bw}{\overline{\w}}
\newcommand{\bv}{\overline{\v}}


\newcommand{\vp}{\bm{\nu}_P^*}
\newcommand{\vu}{\bm{\nu}^u}
\newcommand{\vuu}{\bm{\nu}^u_{S^{\setminus}}}
\newcommand{\vn}{\bm{\nu}_{S}^*}
\newcommand{\vnu}{\bm{\nu}_{S^{\setminus}}^*}

\newcommand{\wuu}{\bm{\omega}^u_{S^{\setminus}}}
\newcommand{\wu}{\bm{\omega}^u}
\newcommand{\vdelta}{\bm{\delta}}
\newcommand{\wt}{\bm{\omega}_{t}}
\newcommand{\wtpp}{\bm{\omega}_{t+1}}
\newcommand{\wk}{\bm{\omega}^{k-1}}
\newcommand{\wkpp}{\bm{\omega}^{k}}
\newcommand{\wtk}{\bm{\omega}_t^{k-1}}
\newcommand{\x}{\vect{x}}
\newcommand{\y}{\vect{y}}
\newcommand{\z}{\vect{z}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}

% \newcommand{\FS}{F_{\tens{S}}}
\newcommand{\FE}{F_{\mathbb{E}}}

\newcommand{\WS}{{\tt W}_S}
\newcommand{\WSU}{{\tt W}_{S^{\setminus}}}

\newcommand{\VS}{{\tt V}_S}
\newcommand{\VSU}{{\tt V}_{S^{\setminus}}}


% \newcommand{\vw}{\bm{\omega}}
% \newcommand{\vv}{\bm{\nu}}

\newcommand{\RA}{\bm{\mathcal{A}}}


% \newcommand{\tU}{\tilde{\U}_t}
% \newcommand{\tV}{\tilde{\V}_t}
% \newcommand{\tX}{\tilde{\X}}
% \newcommand{\tY}{\tilde{\Y}}
% \newcommand{\tx}{\tilde{\x}}
% \newcommand{\ty}{\tilde{\y}}

% \renewcommand{\L}{\mathcal{L}}

\newcommand{\cn}{\kappa}
\newcommand{\nn}{\nonumber}
\newcommand{\order}[1]{O(#1)}
% \newcommand{\M}{\mat{M}}
% \newcommand\Mmh{\mat{M}^{-1/2}}
% \newcommand{\A}{\mat{A}}
% \newcommand{\B}{\mat{B}}
% \newcommand{\C}{\mat{C}}
% \newcommand{\Et}[1][t]{\mat{E_{#1}}}
% \newcommand{\Etp}{\Et[t+1]}
% \newcommand{\Errt}[1][t]{\mat{\bigtriangleup_{#1}}}
% \newcommand\cnM{\kappa}
% \newcommand{\cn}[1]{\kappa\left(#1\right)}
% \newcommand\X{\mat{X}}
% \newcommand\fstar{f_*}
% \newcommand\Xt[1][t]{\mat{X_{#1}}}
% \newcommand\ut[1][t]{{u_{#1}}}
% \newcommand\Xtinv{\inv{\Xt}}
% \newcommand\Xtp{\mat{X_{t+1}}}
% \newcommand\Xtpinv{\inv{\left(\mat{X_{t+1}}\right)}}
% \newcommand\U{\mat{U}}
% \newcommand\UTr{\trans{\mat{U}}}
% \newcommand{\Ut}[1][t]{\mat{U_{#1}}}
% \newcommand{\Utinv}{\inv{\Ut}}
% \newcommand{\UtTr}[1][t]{\trans{\mat{U_{#1}}}}
% \newcommand\Utp{\mat{U_{t+1}}}
% \newcommand\UtpTr{\trans{\mat{U}_{t+1}}}
% \newcommand\Utptild{\mat{\widetilde{U}_{t+1}}}
% \newcommand\Us{\mat{U^*}}
% \newcommand\UsTr{\trans{\mat{U^*}}}
% \newcommand{\Sigs}{\mat{\Sigma}}
% \newcommand{\Sigsmh}{\Sigs^{-1/2}}
% \newcommand{\eye}{\mat{I}}
% \newcommand{\twonormbound}{\left(4+\DPhi{\M}{\Xt[0]}\right)\twonorm{\M}}
% \newcommand{\lamj}{\lambda_j}

% \renewcommand\u{\vect{u}}
% \newcommand\uTr{\trans{\vect{u}}}
% \renewcommand\v{\vect{v}}
% \newcommand\vTr{\trans{\vect{v}}}
% \newcommand\w{\vect{w}}
% \newcommand\wTr{\trans{\vect{w}}}
% \newcommand\wperp{\vect{w}_{\perp}}
% \newcommand\wperpTr{\trans{\vect{w}_{\perp}}}
% \newcommand\wj{\vect{w_j}}
% \newcommand\vj{\vect{v_j}}
% \newcommand\wjTr{\trans{\vect{w_j}}}
% \newcommand\vjTr{\trans{\vect{v_j}}}

% \newcommand{\DPhi}[2]{\ensuremath{D_{\Phi}\left(#1,#2\right)}}
% \newcommand\matmult{{\omega}}



